A Framework for Finding Local Saddle Points in Two-Player Zero-Sum Black-Box Games

Saddle point optimization is a critical problem employed in numerous real-world applications, including portfolio optimization, generative adversarial networks, and robotics. It has been extensively studied in cases where the objective function is known and differentiable. Existing work in black-box settings with unknown objectives that can only be sampled either assumes convexity-concavity in the objective to simplify the problem or operates with noisy gradient estimators. In contrast, we introduce a framework inspired by Bayesian optimization which utilizes Gaussian processes to model the unknown (potentially nonconvex-nonconcave) objective and requires only zeroth-order samples. Our approach frames the saddle point optimization problem as a two-level process which can flexibly integrate existing and novel approaches to this problem. The upper level of our framework produces a model of the objective function by sampling in promising locations, and the lower level of our framework uses the existing model to frame and solve a general-sum game to identify locations to sample. This lower level procedure can be designed in complementary ways, and we demonstrate the flexibility of our approach by introducing variants which appropriately trade off between factors like runtime, the cost of function evaluations, and the number of available initial samples. We experimentally demonstrate these algorithms on synthetic and realistic datasets in black-box nonconvex-nonconcave settings, showcasing their ability to efficiently locate local saddle points in these contexts.

==> figures_latex/main_scenario.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
   \includegraphics[width=0.5\textwidth]{images/obj.png}
% \vspace{-1.0em}
\caption{\textbf{Motivating Example:} }
\label{fig:motivating_example}
% \vspace{-3.5em}
\end{wrapfigure}


==> figures_latex/method_overview.tex <==
\begin{figure*}
    \centering  
    \begin{subfigure}[b]{0.71\textwidth}  
        \includegraphics[width=\textwidth,scale=2]{images/bsp_overview.png}
        \caption{An overview of the high-level game.} 
        \label{fig:bsp_overview}  
    \end{subfigure}  
    \begin{subfigure}[b]{0.68\textwidth}  
        \includegraphics[width=\textwidth,scale=2]{images/llgame_overview.png}  
        \caption{An overview of the low-level game.} 
        \label{fig:llgame_overview}    
    \end{subfigure}
    \caption{
    \todo{saddle point of mean function}
    \hmzh{Overviews of the high-level and low-level games. We include annotations, particularly in \cref{fig:llgame_overview}, that highlight the variant algorithms described in \cref{subsec:alt_alg}.}}
\end{figure*}  

==> figures_latex/obj_cvx_cn.tex <==
\begin{figure*}
    \centering  
    \begin{subfigure}[b]{0.49\textwidth}  
        \includegraphics[width=\textwidth,scale=2]{images/obj_cvx_cvn.png}  
        \caption{\todo{remove}\todo{replace with other exponential example}Convex-concave objective landscape.} 
        \label{fig:cvx_obj}  
    \end{subfigure}  
    \begin{subfigure}[b]{0.49\textwidth}  
        \includegraphics[width=\textwidth,scale=2]{images/poly_obj_landscape_ucb_lcb_init.png}  
        \caption{\todo{remove}Complex polynomial objective landscape.} 
        \label{fig:poly_obj}    
    \end{subfigure}
    \caption{Objective Landscapes}
\end{figure*}  

==> figures_latex/qual_plot.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{images/obj_landscape_ucb_lcb_seed2.png}
        \caption{\textbf{Predicted UCB and LCB}}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{images/obj_landscape_ucb_lcb_newton_seed2.png}
        \caption{\textbf{Newton Descent on a sample problem}}
    \end{minipage}
\end{figure*}

==> figures_latex/random_zero.tex <==
\begin{figure*}
 \begin{center}
    \includegraphics[width=1\textwidth]{images/baselines.png}
    \end{center}
    \caption{ \todo{regenerate figure}
\textbf{Our Bayesian Saddle Point (BSP) methods (orange and green) outperform the baselines of random sampling (purple) and zeroth-order finite difference methods (pink).} The horizontal axis denotes the number of underlying function evaluations, while the vertical axis represents the value of the real merit function, $M^f$.
}
\label{fig:random-zero}
\end{figure*}

==> sections/old/intro.tex <==
\section{Introduction}

Saddle point optimization \cite{Tind2009} is widely used in various real-world applications in economics \cite{luxenberg2022robust}, machine learning \cite{goodfellow2020generative}, robotics \cite{agarwal2023robust}, communications \cite{Moura2019Game}, chemistry \cite{Henkelman2000climbing}, and more.
% Saddle point optimization, 
Also referred to as a two-player zero-sum game, it involves finding a point in the optimization landscape that simultaneously represents a minimum in one direction and a maximum in another.

Saddle point optimization has been widely studied for known and differentiable objective functions; however, this assumption does not encompass numerous real-world situations where the objective is unknown or non-differentiable and can only be sampled.
Such objectives are often referred to as black-box.
For example, in robust portfolio optimization, the goal is to create portfolios resistant to stock market fluctuations \cite{nyikosa2018afinance}, which are inherently random and difficult to model but can be sampled in a black-box fashion through trial and error.
Similar problems arise in various physical systems, such as robotics \cite{lizotte2007robotics} and communication networks \cite{qureshi2023communication}.
% \david{good to have some cites for these examples}
% seek a solution where the trading algorithm is robust to stock market fluctuations

Motivated by these real-world examples, we present a framework for solving saddle point optimization problems in the black-box setting. 
While previous research has primarily focused on solving minimax problems in black-box settings, to our knowledge, none have specifically addressed saddle point problems.
The main distinction between these two types of optimization lies in their respective objectives: saddle point optimization seeks a point that is simultaneously a minimum in one direction and a maximum in another, while minimax optimization aims to find a point that minimizes the worst-case outcome.
In particular, our proposed method strives to identify a saddle point, $(x^*, y^*)$, such that $f(x^*, y) \leq f(x^*, y^*) \leq f(x, y^*)$, for all $x, y$ in the domain.
Although finding global saddle points remains an open problem in general settings, our work focuses specifically on discovering local saddle points, as detailed in \cref{remark:saddle_point}.
To the best of our knowledge, our work is the first to pursue such a solution in a black-box setting.
\hmzh{Moreover, proposing a framework enables our method improve performance in use cases with different accuracy and runtime requirements or cost of evaluation.}



==> sections/old/method.tex <==
\section{Black-box Algorithms for Finding Local Saddle Points}

% \david{
    % do you think we could add a banner across the top that has a flow chart of the general structure of the approach? 
    % I think this section currently is going to lose people. 
    % for example, we are spending as much talking about Newton's method (which is not our contribution, obviously) 
    % as we are about the setup of the high level game, and 
    % nowwhere in the front of this section do we adequately describe the full framework. it was alluded to earlier but needs to be front and center here
% }
We present our approach for identifying local saddle points for the black-box setting, as detailed in \cref{sec:formulation}.
Given that the function, $f$, is unknown, we model it using a \ac{gp}, as described in \cref{subsec:gaussian_process}.
We build a new \ac{bo}-inspired framework to locate the local saddle points.

% Our method involves a sequential search for the saddle point, beginning with an initial prior over $f$.
% Consequently, we seek a local saddle point, such that \cref{def:local_nash_point_2player} with the acquisition function as the cost function.  
% \begin{equation} \label{eq:bo_saddle_opt}
%     x^*, y^* =  \argmin_x \argmax_y \phi(x, y) = \argmax_y \argmin_x \phi(x, y).
% \end{equation}

% We begin with an overview of our method. 
We propose a bilevel algorithm and refer to its component parts as the \textit{low-level} and \textit{high-level} games.
We frame the problem of finding local saddle points for an unknown objective function as a two-level procedure as follows.
The low-level game is general-sum and its solutions are local Nash points which are found by searching for the roots of a system of nonlinear algebraic equations.
The high-level game is zero-sum, and we solve it for local saddle points by first querying the point returned by the low-level game to refine the \ac{gp} around it. Then, the high-level game verifies the Nash point's validity as a local saddle point according to whether it satisfies first-order necessary conditions, \cref{prop:first_order_necessary_condition}, for the \ac{gp} mean.
% We depict our method in \cref{fig:bsp_overview} and \cref{fig:llgame_overview}. 

% \input{figures_latex/method_overview}

% % \david{yeah i think this structure (if not the full rationale) needs to come earlier} 
% \hmzh{The \textit{low-level} algorithm solves a general-sum game 
% % \cref{eq:generalsumgame}
% for a local Nash point using a nonlinear root-finder}.
% The \textit{high-level} game is a zero-sum game with the mean function, $\mu$, as the objective and it searches for a local saddle point.
% We employ the \textit{low-level} game as a \todo{sub-routine} within the solver of the \textit{high-level} game.
% To confirm whether a local Nash point is a local saddle point, we verify whether the solution to the low-level game satisfies the first-order necessary conditions, \cref{prop:first_order_necessary_condition}, for the high-level zero-sum game, i.e., when players have the opposite objectives.
% We depict our method in \todo{Add figures!}.
% }

% \david{maybe i am just feeling grumpy, but i think this reads a bit too ad hoc and reviewers or other readers might smell blood. I would try to rephrase this bit to sound more principled and less like ``we had some intuition and just tried something.'' it's a matter of strategic phrasing more than anything else}

\hmzh{Because the initial prior over $f$ may be a noisy and potentially inaccurate estimate of $f$, we select our optimization strategy for solving the low-level game to encourage exploration.
Specifically, we formulate our low-level problem as a general-sum game with differing objectives: one player minimizes the $\lcb$ and the other maximizes the $\ucb$:}
\begin{equation} \label{eq:generalsumgame}
    \begin{aligned}
        \textsc{Player 1:}& \quad \bar{x}^* = \argmin_x \lcb_t(x, y) \hspace{1em} \textsc{Player 2:}& \quad \bar{y}^* = \argmax_y \ucb_t(x, y).
    \end{aligned}
\end{equation}
\hmzh{The confidence bounds are iteratively constructed and updated within the high-level game as we gather samples of $f(x, y)$ and utilized within each call to the low-level game.
We use the subscript $t$ to indicate the confidence bounds at iteration $t$ of the high-level game.
These choices for each player's objective promote exploration within each iterative update by identifying conservative solutions where the \ac{gp} is uncertain, i.e. has a high $\ucb$ and a low $\lcb$. }
% which conservatively reduce 
% that account for as much uncertainty captured by the bounds $\lcb_t$ and $\ucb_t$ to the zero-sum objective $f$ around $(x, y)$.}
\hmzh{We assume that at least one Nash point exists for the general-sum game at any given iteration so that there is a solution.}
The solution, $(\bar{x}^*, \bar{y}^*)$, of the general-sum game
% \david{readers may wonder about existence. let's discuss how to treat this issue}
will be a local Nash point and should satisfy the first-order necessary conditions in \cref{prop:first_order_necessary_condition}, specifically, $\nabla_{\bar{x}^*} \mathrm{LCB}_t(\bar{x}^*, \bar{y}^*) = 0 $ and $\nabla_{\bar{y}^*} \mathrm{UCB}_t(\bar{x}^*, \bar{y}^*) = 0$.
We formulate the problem of searching for such a point as a nonlinear root-finding problem and use first-order conditions on $\lcb_t$ and $\ucb_t$ to extract local Nash points of the confidence bounds for the general-sum game in \cref{eq:generalsumgame}.

In the high-level game, we seek to solve a zero-sum game to identify the saddle points of $\mu_t$, the mean function of the \ac{gp} at iteration $t$,
% \todo{Distinuish the solution notations to each game $\hat{x}_t$?.}
\begin{equation} \label{eq:zerosumgame}
    \begin{aligned}
       (x^*, y^*) = \argmin_x \argmax_y \mu_t(x, y).
    \end{aligned}
\end{equation}
\hmzh{Upon extracting a solution to the general-sum game in the low-level game, the high-level game can perform additional sampling of the objective around the low-level Nash point $(\bar{x}^*, \bar{y}^*)$.
The results of this sampling is used to update the bounds $\lcb_t$ and $\ucb_t$ at each iteration of the high-level game.
Critically, our method relies on the observation that any solution that satisfies the first-order conditions \cref{prop:first_order_necessary_condition} for $\mu_t$, specifically $\nabla_{x^*} \mu_t(x^*, y^*) = 0$ and $\nabla_{y^*} \mu_t(x^*, y^*) = 0$, will be a saddle point for the mean function since the minimization and maximization objectives are equivalent.
}

% Specifically, we promote exploration  which can conservatively reducing the uncertainty captured by the bounds
% To minimize the objective, we use $\lcb$, and to maximize the objective, we apply the $\ucb$, as in \cref{eq:ucb}.
% Intuitively, the regions with high variance will have lower values in $\lcb_t$ and higher values in $\ucb_t$, thus promoting exploration which can conservatively reducing the uncertainty captured by the bounds.
% Since these optimization objectives are different, we formulate our problem as a general-sum game:

% Each iterative update adjusts the confidence bounds minimally, considering the least-bad adjustment.}
% Our game formulation, \cref{eq:generalsumgame}, naturally accommodates the presence of uncertainty by assigning objectives that promote exploration. \david{didn't this point just get made? feels too soon to repeat} 


% \hmzh{We motivate our proposed algorithms with a key observation: as the bounds $\lcb_t$ and $\ucb_t$ 
% Any root of $G_t^{\mathrm{CB}}$ will be a local Nash point of the confidence bounds since we are solving a general-sum game in \cref{eq:generalsumgame}. 
% Following this observation, w


% \subsection{Solving The Low-Level Game}
\subsection{Nonlinear Root-finding} 
We begin by introducing a new function, $G_t^{\mathrm{CB}}(x, y) : D \times D \rightarrow \mathbb{R}^{k}$, such that its roots satisfy the first-order conditions, \cref{prop:first_order_necessary_condition}, of a local saddle point. Specifically, we seek the roots of the following nonlinear system of (algebraic) equations:
\begin{equation}
G_t^{\mathrm{CB}}(x, y) = \left[\begin{array}{c} \nabla_{x} \lcb_t (x, y) \\  -\nabla_{y} \ucb_t (x, y) \end{array}\right] = 0.
\end{equation}
The superscript $\mathrm{CB}$ signifies that we are finding the roots with confidence bounds (CB) as the objective, while the subscript $t$ denotes the confidence bounds at iteration $t$. To find the roots of $G_t^{\mathrm{CB}}(x, y)$, we employ Newton's method, which is an iterative method that is widely utilized for solving nonlinear systems. Newton's step, $p_t(x, y)$, for root finding is obtained by linearly approximating the function, $G_t^{\mathrm{CB}}$, at the current estimate $(x, y)$ and identifying root of that approximation. The step $p_t(x, y)$ therefore satisfies:
% A Newton step satisfies: \david{give me (in words, and equations) the second line of (8) before you tell me about the step $p$} \david{what is the hat doing on x, y?} \david{this is indicating that you do not linesearch. is that accurate?}
\begin{align} \label{eq:newton_eq}
    \begin{split}
        J_t(x, y) p_t(x, y) = - G_t^{\mathrm{CB}}(x, y),
        % \left[\begin{array}{c} \hat{x} \\ \hat{y} \end{array}\right] = \left[\begin{array}{c} x \\ y \end{array}\right]  + p_t(x, y).
    \end{split}
\end{align}
where $J_t(x, y)$ is the Jacobian matrix of $G_t^{\mathrm{CB}}(x, y)$ calculated as
\begin{equation} \label{eq:hessian}
J_t(x, y) =\left[\begin{array}{cc} \nabla_{x,x}^2 \lcb_t  & \nabla_{x,y}^2 \lcb_t \\ - \nabla_{y,x}^2 \ucb_t & - \nabla_{y,y}^2 \ucb_t \end{array}\right].
\end{equation}
Consequently, we update the current point, $(x, y)$, by taking the step $p_t$ to reach the next point. In our experiments, we employ Newton's method with line search, which is known to converge rapidly when initialized near a root, as shown in \cite[Chpt. 11]{nocedal2006numerical}. Note that the Jacobian $J_t$ requires minimal effort to compute in the lower-dimensional spaces that are classically amenable to black-box optimization.
% \david{should bring this up earlier as well in the related work. don't let a reader ever think we were going to be solving high dimensional problems}.
We provide exact implementation details in \cref{appendix:exper_dets}.

To gauge the progress towards a root of $G_t^{\mathrm{CB}}(x, y)$, we will employ a \textit{merit function}, a scalar-valued function of $(x, y)$, which equals zero at a root and grows unbounded far away from a root. Specifically, we will use the sum of squares as the merit function, defined by:
\begin{equation} \label{eq:merit}
M_t^{\mathrm{CB}}(x, y) = \frac{1}{2} || G_t^{\mathrm{CB}}( x, y) ||_2^2.
\end{equation}
Given that $M_t^{\mathrm{CB}}(x^*, y^*) \geq 0$ for all $(x, y)$, each root serves as a global minimizer of $M$.

\subsection{Local Nash Point to Local Saddle Point} \label{subsec:local_to_saddle}

% \david{this observation needs to occur earlier, far closer to when you first introduce the general-sum inner game (which is currently not explicitly introduced, but should be). i am saying this to emphasize the `why' $\to$ `what' $\to$ `how' principle}
Our proposed algorithms
% , which we will describe in the next section, 
are motivated by a key observation, that any root of $G_t^{\mathrm{CB}}$ will be a local Nash point of the confidence bounds since we are solving a general-sum game in \cref{eq:generalsumgame}. 
% To confirm if a point is a local saddle point, we need to verify if the point satisfies the first-order necessary conditions, \cref{prop:first_order_necessary_condition}, for a zero-sum game, i.e., when players have the opposite objectives. Following this observation, we will construct an algorithm in two parts, referred to as \textit{low-level} game and \textit{high-level} game. \david{yeah i think this structure (if not the full rationale) needs to come earlier} We employ the \textit{low-level} game as a sub-routine within the \textit{high-level} game. The \textit{low-level} will be a general-sum game and will aim to find a local Nash point of \cref{eq:generalsumgame}. The \textit{high-level} game will be a zero-sum game with the mean function, $\mu$, as the objective and will search for its local saddle point. 
For the high-level game, we define a new root function $G_t^{\mu}$ and the corresponding \textit{merit} function, $M_t^{\mu}$, as:
\begin{equation} \label{eq:bsp_root_merit}
    G_t^{\mu}(x, y) = \left[\begin{array}{c} \nabla_{x} \mu_t (x, y)  \\ \nabla_{y} \mu_t (x, y) \end{array}\right], \quad M_t^{\mu} = \frac{1}{2} ||G_t^{\mu}(x, y) ||^2.
\end{equation}
The superscript $\mu$ denotes that we are finding the roots with the mean function, $\mu_t(x, y)$, as the objective. These alternate versions are motivated by the fact that any root of $G_t^{\mu}$ will be a saddle point for the mean function since the minimization and maximization objectives are equivalent.

% \david{meta comment: I wish you would put this architecture right after (5), because only with this structure in mind does it even make sense to be talking about UCBs and LCBs.}
% \edits{I think about it differently. Using UCB and LCB is the most natural thing to do. However, that won't give you saddle points. So first, we present the trivial thing to do and show what the problem is with that and present the solution for that problem.}

 % Additionally, since we have sampled at this point, we have decreased the variance at that point, and thus the mean $\mu_t (x, y)$ is a good representation of the underlying objective function. Additionally, sampling the point allows us to construct better estimators of the gradients at that point. 

% . As such, since $\ucb_t - \lcb_t = 2\beta_t \Sigma_t\left( x, y \right)$, we can show that $\ucb_t = \lcb_t$ by minimizing the variance, $\Sigma_t\left( x, y \right)$, at the point $(x, y)$. This leads to our second key insight: we can minimize the variance at a point by sampling the underlying objective at that point. In the case of no observation noise, $z_t = 0$, we have $\Sigma_t\left( x, y \right) = 0$ for a sampled point $(x, y)$. However, in the case of observation noise $z_t \sim \mathcal{N}\left(0, \sigma^2\right)$, this is not true. As such, we introduce alternate versions of the root function $G_t$ and the \textit{merit} function $M_t$, referred to as $G_t^{\ac{bsp}}$ and $M_t^{\ac{bsp}}$:

% We formalize the fact that $\ucb_t = \lcb_t$ after sampling in \cref{lemma:zero_noise,lemma:with_noise}.
% \begin{lemma}[Local Nash Point is Local Saddle Point after sampling] \label{lemma:with_noise}
% For given $\ucb_t$ and $\lcb_t$, and the root $(\bar{x}^*, \bar{y}^*)$ of $G_t$, the root $(\bar{x}^*, \bar{y}^*)$ and therefore \textit{high-level} game will be a zero-sum game. \david{grammar. also is this true? certainly not with measurement noise.}
% \end{lemma}

% The \textit{high-level} game employs $G_t^{\ac{bsp}}, M_t^{\ac{bsp}}$, while the \minigame \space uses $G_t$, $M_t$ in \cref{alg:bsp,alg:low_level_game} respectively. This minor modification ensures that the \textit{high-level} game is a zero-sum game, and its solution will be a local saddle point. In \cref{lemma:with_noise}, we show that after sampling the point $(\bar{x}^*, \bar{y}^*)$ (the output of \cref{alg:low_level_game}), we achieve $\ucb_t = \lcb_t$. The main insight is that the final point returned by \cref{alg:low_level_game} should not be treated as a local saddle point; instead, we must query $f$ to verify whether the local saddle point has indeed been reached.


\subsection{Finding Local Saddle Points with \ac{bsp}}
% : A Two-Level Game 

We present our algorithm for finding local saddle points, which we will refer to as \ac{bsp}. 

In \cref{alg:low_level_game}, we present our \textit{low-level} game, which we refer to as \minigame.
\minigame \space utilizes the current confidence bounds, $(\lcb_{t}, \ucb_{t})$, to determine the local Nash points by finding roots of $G_t^{\mathrm{CB}}$ using Newton's method.
The \minigame \space function does not make any new queries of $f$; instead, it uses the most updated confidence bounds to identify the local Nash points.
The function takes an initial point, $(x, y)$, and current confidence bounds, $(\lcb_{t}, \ucb_{t})$, as inputs.
Starting from line 2, the function iteratively updates the point, $(\bar{x}_t, \bar{y}_t)$, using \cref{eq:newton_eq} and halts when the merit function, $M_t^{\mathrm{CB}}(\bar{x}_t, \bar{y}_t)$, is sufficiently small. Consequently, the while loop terminates when gradients $\nabla_{\bar{x}_t} \lcb_t (\bar{x}_t, \bar{y}_t)$ and $ \nabla_{\bar{y}_t} \ucb_t(\bar{x}_t, \bar{y}_t)$ are sufficiently small. Ultimately in line 4, the function returns the final point, $(\bar{x}^*, \bar{y}^*)$, once it discovers a local Nash point.

\input{figures_latex/algo}

We now present \cref{alg:bsp}, which searches for the local saddle points. As stated earlier, this distinction between the two games allows us to confirm if a local Nash point is a local saddle point. In \cref{alg:bsp}, we start by optimizing the hyperparameters of our \ac{gp} kernel using the initial dataset, $\mathcal{S}_0$, a standard procedure in \ac{bo} \cite{Snoek2012practical}. Upon learning the hyperparameters, an initial GP prior, $(\mu_0, \sigma_0)$, is obtained. Then in line 1, we select a starting point, $(x_0, y_0)$, from the initial dataset, $\mathcal{S}_0$, based on the lowest \textit{merit} value. From this point, an iterative search for the local saddle point is conducted in the outer while loop (lines 2-6). The \minigame \space function is utilized in line 3 to determine the subsequent point $(x_{t+1}, y_{t+1})$, which is a local Nash point of the general-sum game \cref{eq:generalsumgame}. The point, $(x_{t+1}, y_{t+1})$, is only a local Nash point for the given $\lcb_t$ and $\ucb_t$; we will not be sure if it is a local saddle point of $f$ until we sample $f$ at that point and calculate $M_t^\mu$ to validate the conditions in \cref{prop:first_order_necessary_condition}. 

Consequently, in line 4, the point returned by \minigame \space is sampled and added to the current dataset. In line 5, new hyperparameters are learned from dataset $\mathcal{S}_{t+1}$, and $\mu_{t+1}, \sigma_{t+1}, \lcb_{t+1}, \ucb_{t+1}$ are updated accordingly.\footnote{This is a standard procedure in black-box optimization, explained in further detail in \cref{appendix:hyper_update}.} After sampling at the point $(x_{t+1}, y_{t+1})$, we have decreased the variance at that point, and thus the mean, $\mu_t(x_{t+1}, y_{t+1})$, is a better representation of $f$. Additionally, sampling the point allows us to construct better estimators of the gradients at that point. As such, we will check if the merit function value is sufficiently small, with $M_t^{\mu}(x_t, y_t) \leq \epsilon$. As the value of $f(x_t, y_t)$ has been observed, $M_t^{\mu}$ is a good estimator if the saddle point has been reached. Ultimately in line 7, the local saddle point $(x^*, y^*)$ is returned after the completion of the outer loop.
% As we sample more points, we hope that the confidence bounds $\lcb$ and $\ucb$ will accurately estimate underlying function $f$ and eventually reach the local saddle point.

\hmzh{To the best of our knowledge, no existing method specifically addresses nonconvex saddle point optimization in a black-box setting.
The most prevalent method is the gradient ascent-descent method ~\cite{lin2020gradient, Mazumdar2019OnFL, adolphs2019local}, which takes gradient steps for minimization and maximization objectives, as opposed to our method's Newton steps.
Additionally, if we apply $\ucb/\lcb$ to the optimization objectives of these methods, as we did in our method, \hmzh{the solutions to} their methods would 
% essentially \david{too imprecise of a word for this discussion} 
solve general-sum games
% . Consequently, the point returned by these methods would be a 
for Nash points rather than saddle points.
As such, our higher and lower game structure can be combined with other algorithms, like the gradient ascent-descent method, to identify local saddle points in black-box settings, highlighting the usefulness and adaptability of our proposed framework.}

% \vspace{-1.5em}

% Although the assumption made in \cref{lemma:convergence} may not be satisfied experimentally, it provides insight into \cref{alg:low_level_game}'s convergence.

\subsection{Convergence} \label{subsec:convergence}

In \cref{lemma:convergence}, we demonstrate that \cref{alg:low_level_game} will terminate and converge to a local Nash point under standard technical assumptions. Our experiments in \cref{sec:experiments} include cases that both satisfy and violate these assumptions, showcasing the performance of our algorithm under various circumstances.

\begin{lemma}[Convergence to Local Nash Point in \minigame] \label{lemma:convergence} \cite[Thm 11.6]{nocedal2006numerical}
Let $J(x, y)$ be Lipschitz continuous in a neighborhood $D \times D \subset \mathbb{R}^{k\times k}$ surrounding the sublevel set $\mathcal{L}= \left\{x, y: M_t^{\mathrm{CB}}(x, y) \leq M_t^{\mathrm{CB}}\left(x_0, y_0\right)\right\}$. Assume that both $||J(x, y)||$ and $||G_t^{\mathrm{CB}}(x, y)||$ have upper bounds in $D$. Let the step lengths $\alpha_k$ satisfy the Wolfe conditions \cite[Thm. 3.6]{nocedal2006numerical}. If $||J(x, y)^{-1}||$ has an upper bound, then \cref{alg:low_level_game} will converge and return a root of $G_t^{\mathrm{CB}}(x, y)$. 
\david{this is also a statement about existence, no? if it is, this should be tied into the discussion i raised earlier}
\end{lemma}

% In \cref{alg:bsp}, we sample the underlying function at the local Nash point returned by \cref{alg:low_level_game} to decrease the variance, $\sigma_t$, in the confidence bounds. After sampling and updating the confidence bounds, the mean function, $\mu_t$, becomes a more accurate estimator of the underlying function, $f$, around the sampled local Nash point. Similarly, the gradient of the mean function, $\nabla \mu_t$, will also be a reliable estimator of the true gradient of the unknown function, $\nabla f$. Consequently, $M_t^\mu \approx M^f$, indicating that the merit function based on $M_t^\mu$ will be a good estimator of the original underlying function gradients, denoted by $M^f$. As such, the merit function, $M_t^\mu$, serves as an effective validator of convergence to the local saddle point. As the estimates of the underlying function, $f$, improve with each iteration, the technical arguments mentioned above suggest that the while loop in \cref{alg:bsp} will eventually terminate at a local saddle point.
In \cref{alg:bsp}, we sample $f$ at the local Nash point returned by \cref{alg:low_level_game} to reduce variance, $\sigma_t$, in confidence bounds. This improves the accuracy of the mean function $\mu_t$ and its gradient $\nabla \mu_t$ as estimators for $f$ and its gradient $\nabla f$, around the sampled point. Consequently, the merit function, $M_t^\mu$, effectively validates convergence to the local saddle point, as it closely approximates $M^f$. As estimates improve with iterations, the while loop in \cref{alg:bsp} is expected to terminate at a local saddle point.

\begin{proposition}[\todo{Convergence of Local Nash Points to Local Saddle Points}] \label{prop:convergence_local_nash_to_saddle} 
    \todo{add assumptions for theorem 2, potentially to problem statement - RKHS, bounded RKHS norm, sub gaussian noise, predictable process with field}
    As the number of sampled points $|S_t| \to \infty$, then finding a local Nash point of $\mu_t$ converges to a first-order stationary point of $f$. 
    % Assuming $f_1$ and $f_2$ are differentiable, any local \hmzh{Nash} point satisfies $\nabla_{x} f_1(x, y) =0$ and $\nabla_{y} f_2(x, y) =0$.
\end{proposition}

\textbf{Proof.}
We first use a result from \cite{chowdhury2017kernels} to show that the UCB acquisition function used in the lower-level problem results in $\mu_t$ converging to $f$ at a bounded rate.
Then, we use this result to conclude that when the GP converges, finding local Nash points in the lower-level game result in first-order stationary points of $f$ in the BSP algorithm, which can then be confirmed to be saddle points using second-order conditions. 

Let the RKHS norm on $D$ with symmetric, positive-definite kernel $K$ be bounded by $B \in \mathbb{R}$.
Let $0 < \delta \leq 1$ be the desired probability of successful convergence.
We note that $\{ \bar{x}^*_t, \bar{y}^*_t \}_{t=1}^\infty$, solutions to the lower-level game \cref{eq:generalsumgame}, form a discrete-time process \hmzh{where $(x_t, y_t)$ is $\mathcal{F}_{t-1}$-measurable.} 
\hmzh{Next, we let $\gamma_{t-1}$ be ...}

Thus, using Theorem 2 from \cite{chowdhury2017kernels}, we conclude that, for all $x, y \in D, t \geq 1$, $\mu_t$ converges to $f$ according to the inequality 
\hmzh{Adjust for two inputs, $\sum_t$.}
\begin{equation}
\label{eq:convergence-rate}
|\mu_{t-1}(x) - f(x)| \leq \left( B + R \sqrt{2(\gamma_{t-1} + 1 + \ln(1 / \delta))} \right) \sigma_{t-1}(x).
\end{equation}

Next, we recall that the derivative of a Gaussian process forms a Gaussian process \citep{rasmussen2003gaussian}.
Specifically, we note that $\nabla f \sim GP(\nabla{} \mu, \nabla \sum())$. \todo{two arguments}
Using the same logic as the first part of our proof, we conclude that as $|S_t| \to \infty$, $\nabla \mu_t \to \nabla f$, meaning that additional samples will also cause this GP to converge (\todo{explain}).

As we keep sampling, the variance $\sigma$ approaches the noise variance, $\sigma_z$. As such, we expect that $\nabla \sigma \to 0$ while the derivative process converges.
The definitions of $\lcb, \ucb$ then imply that $\nabla \lcb, \nabla \ucb \to \nabla \mu$ as the variance term is eliminated.

In the final step of this proof, we first recall that solutions to the lower-level game must satisfy the first order conditions $\nabla \lcb = 0, \nabla \ucb = 0$.
As $\nabla \lcb, \nabla \ucb \to \nabla \mu$, we can then note that $\nabla \mu$ reliably estimates $\nabla f$ and thus local Nash solutions to the lower-level game will converge to first-order stationary points of $f$.
If the second-order optimality conditions for a saddle point are met, then the Nash equilibria produced by the lower-level game converge to local saddle points of the higher-level game, as desired.

% \begin{enumerate}
%     \item As we sample local Nash points, the variance in the confidence bounds at that local Nash point will decrease, and $\lcb/\ucb$ will get closer to each other, as discussed in the \cref{appendix:proof}. 
%     \item As we keep sampling, the variance will eventually become the noise variance, $\sigma_z$. As such, $\nabla \sigma \rightarrow 0$ and therefore $\nabla \lcb, \nabla \ucb \rightarrow \nabla \mu$. 
%     \item As stated in the previous paragraph, since $\nabla \mu$ is a reliable estimator of the true gradients of the unknown function, $\nabla f$, finding local Nash points of the confidence bounds will eventually lead to local saddle points of $\mu$ and consequently \hmzh{at least a first-order stationary point} of $f$. 
% \end{enumerate}


We focus on the experimental characterization of this algorithm and its variants as a proof of concept, leaving theoretical convergence analysis for future work. Nevertheless, we provide an intuitive explanation of why sampling at local Nash points of confidence bounds will lead to local saddle points of $f$. As we sample local Nash points, the variance in the confidence bounds at that local Nash point will decrease, and $\lcb/\ucb$ will get closer to each other, as discussed in the \cref{appendix:proof}. As we keep sampling, the variance will eventually become the noise variance, $\sigma_z$. As such, $\nabla \sigma \rightarrow 0$ and therefore $\nabla \lcb, \nabla \ucb \rightarrow \nabla \mu$. As stated in the previous paragraph, since $\nabla \mu$ is a reliable estimator of the true gradients of the unknown function, $\nabla f$, finding local Nash points of the confidence bounds will eventually lead to local saddle points of $\mu$ and consequently \hmzh{at least a first-order stationary point} of $f$. 
% \david{is there a way to make this logic formal and call it a proposition?}


% Specifically at a sampled point, $(x, y)$, in the case of zero observation noise, $z_t = 0$, we show in \cref{remark:zero_noise} that $\lcb(x, y) = \ucb(x, y)$, and in the case of observation noise, $z_t \sim \mathcal{N}\left(0, \sigma_z^2\right)$, we show in \cref{remark:observation_noise} that $\ucb_t(x, y) - \lcb_t(x, y) = 2 \beta \sigma(x, y)$. As such, we believe that our general-sum \minigame \space game will eventually become a zero-sum game.

Finally, the point returned by our proposed algorithm may not always satisfy the second-order sufficient conditions (\cref{prop:second_order_necessary_condition}). As a result, we will verify the second-order condition (\cref{prop:second_order_necessary_condition}) for the final saddle point returned by \cref{alg:bsp} \hmzh{\cite{ratliff2016characterization,balduzzi2018mechanics,mazumdar2020gradient}}. If the final returned point does not satisfy the second-order conditions, we will need to reinitialize our algorithm from a new initial point.
% \david{could point to eric and other subsequent papers to discuss that it remains an open problem to use first- or second-order methods definitively converge to poitns which satisfy second order conditions. there is a paper from Chinchilla and Hespanha which solves it for minimax and may be worth citing. kushagra is working on the saddle point case and may be worth consulting as well}

% Furthermore, since we use Newton's method, we can expect quadratic convergence when we start close to the saddle point, and superlinear convergence in other cases. A detailed convergence analysis of Newton's method can be found in \cite{nocedal2006numerical}.

%   Then we have that the Zoutendijk condition holds, that is,
% $$
% \sum_{k \geq 0} \cos ^2 \theta_k\left\|J_k^T r_k\right\|^2<\infty
% $$
% where
% $$
% \cos \theta_k=\frac{-p_k^T \nabla f\left(x_k\right)}{\left\|p_k\right\|\left\|\nabla f\left(x_k\right)\right\|}
% $$



\subsection{Variants of BSP} \label{subsec:alt_alg}

\textbf{\Ac{bsp} Expensive:} Our \Ac{bsp} method in \cref{alg:bsp} aims to minimize queries of the function $f$ by taking multiple Newton steps per query of $f$.
However, the algorithm may become unstable if the confidence bounds $\ucb_{t+1}, \lcb_{t+1}$ do not accurately approximate $f$.
Additionally, it is possible that querying $f$ can often be inexpensive, for example, in the case of Reinforcement Learning, \cite{sutton2018reinforcement}, in simulation.
In this case, we query $f$ during each iteration of \cref{alg:bsp} after taking a single Newton step, in contrast to the multiple steps taken in \cref{alg:low_level_game} (lines 2-3).
This approach is referred to as \ac{bsp}-\textit{expensive} since we make more queries of $f$, while our original algorithm in \cref{alg:bsp} is referred to as \ac{bsp}-\textit{efficient}. 
\hmzh{We demonstrate in our results that this variant can more effectively and efficiently solve complex scenarios than simpler methods like finite differencing) that become feasible under these conditions.}
% \hmzh{Finite differencing what?}
% \david{if i were a reviewer, i would ask: for the `expensive' case, why use the GP stuff at all and not just do finite differencing? i believe you baselined against this though, right?}

% By querying $f$ more frequently, we can better estimate confidence bounds, $\ucb_{t+1}, \lcb_{t+1}$, resulting in increased stability and quicker convergence, albeit with more queries of $f$.

% 

\textbf{Exploration and Exploitation:} In \cref{alg:bsp}, we encourage more exploration by using $\lcb$ for minimization and $\ucb$ for maximization. Since the value of unexplored regions has high variance and thus a lower $\lcb$ value, the minimization procedure will explore those regions first (vice-versa for $\ucb$ and maximization). As such, we refer to our original proposed method, as \ac{bsp}-\textit{explore}. Alternatively, we can use LCB for maximization and UCB for minimization, thus promoting more exploitation by our algorithm. We will refer to this variant as \ac{bsp}-\textit{exploit}. In real-world scenarios, this approach might be suitable when optimizing a well-understood process, fine-tuning known models, or when domain knowledge allows for confidently focusing on exploitation.

% When UCB/LCB are not accurate approximations of $f$, \ac{bsp}-\textit{conservative} is \david{we have not done the evaluation yet, so i would just forward reference that discussion here} the better choice. This situation can arise when there are insufficient samples to initialize \ac{bo}, leading to poor UCB/LCB approximations. On the other hand, if there are ample samples to initialize \ac{bo}, \ac{bsp}-\textit{optimistic} can be utilized for potentially faster convergence.



% \david{I would probably refactor this paragraph into the experiments section}




% Depending on the confidence of observations of $f$, UCB/LCB approximations, and efficiency requirements, the user can decide which of the three algorithms to use.


% While classical Bayesian optimization (BO) has been shown to be effective in solving a wide range of optimization problems, it is limited by its ability only to identify the maximum (or minimum) of an objective function. In this work, we aim to go beyond classical BO by identifying a saddle point of the unknown objective function $f$. We will model the unknown objective function, denoted by $f$, using the confidence bounds as defined in Section \ref{sec:formulation}.  This approach is commonly employed in the literature, where we are conservative in the face of uncertainty by underestimating both the minimization and maximization objectives. Alternatively, we can flip these to act optimistically, which we discuss further in \cref{subsec:alt_alg}. 

% Since we are minimizing $f$ with respect to $x$, we will use $ \nabla_{x} \ucb_t (x, y)$, the gradient of $\ucb_t$ with respect to minimizing variable $x$. Similarly, since we are maximizing $f$ with respect to $y$, we will use $ - \nabla_{y} \lcb_t (x, y)$, the negative gradient of $\lcb_t$ with respect to maximizing variable $y$.

% . Although the Nash point returned by \minigame, $(\bar{x}^*, \bar{y}^*)$, exhibits $M_t(\bar{x}^*, \bar{y}^*) \leq \epsilon$, it is uncertain whether the local saddle point has been found since the point  the point has not been sampled and the gradients $\nabla_{\bar{x}^*} \ucb_t (\bar{x}^*, \bar{y}^*)$ and $\nabla_{\bar{y}^*} \lcb_t (\bar{x}^*, \bar{y}^*)$ are unknown.

==> sections/old/related_works.tex <==
% \input{figures_latex/main_scenario}

% \subsubsection*{Related Works}
\textbf{\hmzh{Optimizing Gaussian Processes:}} Over the years, a plethora of algorithms have been developed for Gaussian Processes (GP) optimization, including GP-UCB \cite{Srinivas2010Gaussian}, entropy search \cite{Hennig2012Entropy}, predictive entropy search \cite{hernandez2014predictive}, truncated Bayesian optimization \cite{bogunovic2016truncated}, max-value entropy search \cite{wang2017max}, and fast Bayesian optimization \cite{ru2018fast}.
Among these, GP-UCB has been widely used in various settings, including robotics \cite{deisenroth2013gaussian}, chemistry \cite{Westermayr2021Machine}, user modeling \cite{Brochu2010ATO}, and reinforcement learning \cite{cheung2020reinforcement}, to name a few.
In this work, we leverage techniques from GP-UCB to model the underlying objective.

\textbf{Minimax Black-box Optimization:} Recently, there has been growing interest in studying minimax optimization in black-box settings.
Works such as ~\cite{Bogunovic2018Adversarially, Lukas2020Noisy, wang2022zeroth} investigate robust optimization problems for various applications and settings. \citet{curi2021Combining} explored robust model-based reinforcement learning, where the environment is a black-box.
\citet{huang2022accelerated}, proposed an accelerated zeroth-order momentum descent ascent method for black-box minimax optimization.
Despite this progress, none of these methods have specifically addressed the saddle point optimization problem.

\textbf{Saddle Point Optimization:}
Saddle point optimization has long been a prominent research topic in both optimization and game theory literature.
Convex-concave saddle point problems, in particular, have been studied since 1928 \cite{Neumann1928Zur}, with works \cite{Korpelevich1976TheEM, Tseng1995OnLC, Nemirovski2004Prox} demonstrating guaranteed convergence.
In contrast, nonconvex saddle point optimization presents a more challenging problem and currently has only approximate solutions, including \cite{lin2020gradient, adolphs2019local, lin2020near}, among others. 
Saddle point optimization has also been extensively studied from a game theory perspective, specifically formulated as a zero-sum game \cite{baser1998dynamic}.
Methods such as \cite{Mazumdar2019OnFL, Fiez2021GlobalCT} contribute additional insights into this area.
Our work distinguishes itself from these methods by considering cases where the objective function is unknown.

\textbf{Contributions}: First, we propose a two-level framework for finding local saddle points in black-box settings, which aims to satisfy first-order necessary conditions (\cref{prop:first_order_necessary_condition}). Our proposed framework consists of two games: a lower-level game and a higher-level game.
The lower-level game identifies local Nash points (\cref{def:local_nash_point_2player}) of a two-player surrogate game, where a set of algorithms can be used, i.e. first-order or second-order.
The high-level optimizer ensures that the local Nash points are local saddle points of the black box system.
Second, we propose a set of algorithms for the lower-level game, with each variant catering to different real-world cases based on uncertainty and sampling cost.
Our framework allows for versatility in trading off between factors like ease of sampling, and exploration and exploitation.
Third, we experimentally demonstrate our algorithms' effectiveness on synthetic and realistic datasets.
As with prior work, our method is appropriate for lower-dimensional spaces which are classically amenable to black-box optimization.
% \david{suggest being more careful about what is an algorithm, subroutine, variant. the term ``framework'' comes to mind}}


% \textbf{Contributions}: First, propose a two-level procedure for finding local saddle points in the black-box setting, which aims to satisfy the first-order necessary conditions, \cref{prop:first_order_necessary_condition}. A \textit{low-level} game solves for the local Nash points by finding the roots of a system of nonlinear algebraic equations. The \textit{high-level} game solves for the local saddle points by querying the point returned by the \textit{low-level} game and verifying its validity as a local saddle point. Second, using our two-level procedure, we propose a set of black-box algorithms to find local saddle points. Our proposed algorithm variants cater to different real-world use cases, depending on the uncertainty and cost of sampling the objective function. Third, we experimentally demonstrate the ability of our proposed algorithms to effectively find local saddle points on synthetic and real-world datasets.

==> sections/todos.tex <==
% \begin{itemize}
% % \item \todo{use iclr 2025 format}
% % \item \todo{Make references table if enough space.}
% % \item \todo{Make list of improvements for figure labels.}
% % \item \todo{Make figure of how method works if enough space.}
% % \item \todo{[Hamzah] Generate 10D polynomial data with LSS and share with somi.}
% \item \textbf{Data + Results}
% % \item \todo{[Somi] Confirm the parameters used for experiments + fill the ablation study tables.}
% % \item \todo{[Hamzah] Fill in LSS row in table + rename columns/rows to explore/exploit?}
% % \item \todo{[Somi] Tweak figures as needed (ARIMA, legends, appendix, etc.).}
% % \item \todo{[Hamzah] discuss LSS}
% % \item \todo{show plot of which ones converge in LSS (in appendix) - given all points converge, show convergence rates $\to$ statement: ,}

% \item Go through and double check all variants and named and referenced by color properly, and that the facts align with plots.
% % \item \todo{More analysis of success rate table in experiments Runtimes + Success Rates (LSS specifically)}
% % \item \hmzh{finite differencing/number samples - hard to explain}
% \item {Variants caption in appendix}
% % \item \todo{Look over language for the LSS failures}
% % \item \hmzh{- explain why we focus on those here}
% % \item In Figure 1, we present blah for clarity and other two in appendix, and here's discusson of full results.

% \item \textbf{Final editing}
% % \item \todo{[Hamzah] Fix ARIMA plots in powerpoint}
% % \item \todo{[Hamzah/Somi] Update experiments + analysis.}
% % \item \todo{Are we missing any major topics?}
% % \item \todo{Update appendix. }
% \item {Cut length - 1 paragraph?}
% \item {Reread fully.}
% % \item \todo{[David + Kushy] Review}

% \item \textbf{Other}
% \item \hmzh{reviewers might ask: why not use GP - can't use LSS on general sum game - global convergence is still an open challenge (if needed) see david's edit}

% % \item \textbf{Items related to LSS + False Nash points}
% % \item \todo{[Hamzah/Somi] Confirm the method of presenting whether we find a saddle for decaying polynomial, i.e. what counts as success in table.}
% % \item \todo{[Hamzah/Somi if necessary] Regenerate LSS handicapped + replot appropriately.}
% % \item \todo{[Hamzah] Should we add an image of LSS converging to a false Nash point in the appendix?}
% \end{itemize}

Last TODOs:
\begin{itemize}
    \item[DONE]resolve red statements
    \item[somi] read the paper, focusing on the changes in the pink statements.
    \item[DONE] add text explaining why the baselines, success rates are as they are (failing, succeeding, etc.).
\end{itemize}

TODOs:
\begin{itemize}
    \item[DONE] Confirm that text and figures were transferred correctly to the new template.
    \item[DONE] Generate and report results for the other three algorithms in Maheswari et al (all algorithms fail to find saddle points, either exiting the valid region or finding the false saddle at the origin).
    \item[both - DONE] Revise claim/motivation about real-world examples as per the area chair's review? Avoid anything that undermines the claim/motivation.
    \item[discuss] Address concerns about dimensionality and what ``low'' dimensional vs. high dimensional means. Justify our approach.
    \item[discuss - DONE] Further discussion on scalability of GPs
    \item[let's not] Add zeroth-order baseline for ARIMA?
    \item[DONE] Clarify further how convergence is checked
    \item Clarify further how/why our baselines are impressive in the discussion.
    \item Move figures from appendix to main paper (we have 12 pages).
\end{itemize}

Possible TODOs:
\begin{itemize}
    \item[Hamzah still exploring] Broader: Lack of theoretical guarantees
    \item[Hamzah] Generate dataset for stock market portfolio optimization
    \item[Somi] Generate results for portfolio optimization. 
\end{itemize}

\newpage

==> style/old_iclr2025/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> style/old_iclr2025/style2024/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> template/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

